DeepCQ: General-Purpose Deep-Surrogate Framework for Lossy Compression Quality Prediction

Error-bounded lossy compression techniques have become vital for scientific data management and analytics, given the ever-increasing volume of data generated by modern scientific simulations and instruments. Nevertheless, assessing data quality post-compression remains computationally expensive due to the intensive nature of metric calculations. In this work, we present a general-purpose deep-surrogate framework for lossy compression quality prediction (DeepCQ), with the following key contributions: 1) We develop a surrogate model for compression quality prediction that is generalizable to different error-bounded lossy compressors, quality metrics, and input datasets; 2) We adopt a novel two-stage design that decouples the computationally expensive feature-extraction stage from the light-weight metrics prediction, enabling efficient training and modular inference; 3) We optimize the model performance on time-evolving data using a mixture-of-experts design. Such a design enhances the robustness when predicting across simulation timesteps, especially when the training and test data exhibit significant variation. We validate the effectiveness of DeepCQ on four real-world scientific applications. Our results highlight the framework's exceptional predictive accuracy, with prediction errors generally under 10\% across most settings, significantly outperforming existing methods. Our framework empowers scientific users to make informed decisions about data compression based on their preferred data quality, thereby significantly reducing I/O and computational overhead in scientific data analysis.

==> prediction_result.tex <==
% % CR results
% \begin{figure*}[t]
%     \centering
%     \begin{subfigure}{.49\columnwidth}
%         \includegraphics[width=\columnwidth]{Figures/sec-4/qnet_BD_CR.png}
%         \vspace{-18pt}
%         \caption{Baryon density}
%         % \vspace{-9pt}
%         \label{fig:qnet_bd_cr}
%     \end{subfigure}
%     \hfill
%     % \begin{subfigure}{.49\columnwidth}
%     %     \includegraphics[width=\columnwidth]{Figures/sec-4/qnet_DMD_CR.png}
%     %     \vspace{-18pt}
%     %     \caption{Dark matter density}
%     %     % \vspace{-9pt}
%     %     \label{fig:qnet_dmd_cr}
%     % \end{subfigure}
%     % \hfill
%     \begin{subfigure}{.49\columnwidth}
%         \includegraphics[width=\columnwidth]{Figures/sec-4/qnet_CLOUDf48_CR.png}
%         \vspace{-18pt}
%         \caption{CLOUDf48}
%         % \vspace{-9pt}
%         \label{fig:qnet_cloud_cr}
%     \end{subfigure}
%     \hfill
%     % \begin{subfigure}{.49\columnwidth}
%     %     \includegraphics[width=\columnwidth]{Figures/sec-4/qnet_PRECIPf48_CR.png}
%     %     \vspace{-18pt}
%     %     \caption{PRECIPf48}
%     %     % \vspace{-9pt}
%     %     \label{fig:qnet_precip_cr}
%     % \end{subfigure}
%     % \hfill
%     \begin{subfigure}{.49\columnwidth}
%         \includegraphics[width=\columnwidth]{Figures/sec-4/qnet_RTM420_CR.png}
%         \vspace{-18pt}
%         \caption{{RTM}}
%         % \vspace{-9pt}
%         \label{fig:qnet_seis_cr}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{.49\columnwidth}
%         \includegraphics[width=\columnwidth]{Figures/sec-4/qnet_633_CR.png}
%         \vspace{-18pt}
%         \caption{{Density}}
%         % \vspace{-9pt}
%         \label{fig:qnet_density_cr}
%     \end{subfigure}
%     \hfill
%     \vspace{-9pt}
%     \caption{CR prediction.\texttt{\_o} and \texttt{\_p} represent the ground truth and predicted values, respectively.}
%     \vspace{-5pt}
%     \label{fig:cr_pred}
% \end{figure*}

% % PSNR results
% \begin{figure*}[t]
%     \centering
%     \begin{subfigure}{.49\columnwidth}
%         \includegraphics[width=\columnwidth]{Figures/sec-4/qnet_BD_PSNR.png}
%         \vspace{-18pt}
%         \caption{Baryon density}
%         % \vspace{-9pt}
%         \label{fig:qnet_bd_psnr}
%     \end{subfigure}
%     \hfill
%     % \begin{subfigure}{.49\columnwidth}
%     %     \includegraphics[width=\columnwidth]{Figures/sec-4/qnet_DMD_PSNR.png}
%     %     \vspace{-18pt}
%     %     \caption{Dark matter density}
%     %     % \vspace{-9pt}
%     %     \label{fig:qnet_dmd_psnr}
%     % \end{subfigure}
%     % \hfill
%     \begin{subfigure}{.49\columnwidth}
%         \includegraphics[width=\columnwidth]{Figures/sec-4/qnet_CLOUDf48_PSNR.png}
%         \vspace{-18pt}
%         \caption{CLOUDf48}
%         % \vspace{-9pt}
%         \label{fig:qnet_cloud_psnr}
%     \end{subfigure}
%     \hfill
%     % \begin{subfigure}{.49\columnwidth}
%     %     \includegraphics[width=\columnwidth]{Figures/sec-4/qnet_PRECIPf48_PSNR.png}
%     %     \vspace{-18pt}
%     %     \caption{PRECIPf48}
%     %     % \vspace{-9pt}
%     %     \label{fig:qnet_precip_psnr}
%     % \end{subfigure}
%     % \hfill
%     \begin{subfigure}{.49\columnwidth}
%         \includegraphics[width=\columnwidth]{Figures/sec-4/qnet_RTM420_PSNR.png}
%         \vspace{-18pt}
%         \caption{{RTM}}
%         % \vspace{-9pt}
%         \label{fig:qnet_seis_psnr}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{.49\columnwidth}
%         \includegraphics[width=\columnwidth]{Figures/sec-4/qnet_633_PSNR.png}
%         \vspace{-18pt}
%         \caption{{Density}}
%         % \vspace{-9pt}
%         \label{fig:qnet_density_psnr}
%     \end{subfigure}
%     \hfill
%     \vspace{-9pt}
%     \caption{PSNR prediction. \texttt{\_o} and \texttt{\_p} represent the ground truth and predicted values, respectively.}
%     \vspace{-5pt}
%     \label{fig:psnr_pred}
% \end{figure*}

% % SSIM
% \begin{figure*}[t]
%     \centering
%     \begin{subfigure}{.49\columnwidth}
%         \includegraphics[width=\columnwidth]{Figures/sec-4/qnet_BD_SSIM.png}
%         \vspace{-18pt}
%         \caption{Baryon density}
%         % \vspace{-9pt} s 
%         \label{fig:qnet_bd_ssim}
%     \end{subfigure}
%     \hfill
%     % \begin{subfigure}{.485\columnwidth}
%     %     \includegraphics[width=\columnwidth]{Figures/sec-4/qnet_DMD_SSIM.png}
%     %     \vspace{-18pt}
%     %     \caption{Dark matter density}
%     %     % \vspace{-9pt}
%     %     \label{fig:qnet_dmd_ssim}
%     % \end{subfigure}
%     % \hfill
%     \begin{subfigure}{.49\columnwidth}
%         \includegraphics[width=\columnwidth]{Figures/sec-4/qnet_CLOUDf48_SSIM.png}
%         \vspace{-18pt}
%         \caption{CLOUDf48}
%         % \vspace{-9pt}
%         \label{fig:qnet_cloud_ssim}
%     \end{subfigure}
%     \hfill
%     % \begin{subfigure}{.485\columnwidth}
%     %     \includegraphics[width=\columnwidth]{Figures/sec-4/qnet_PRECIPf48_SSIM.png}
%     %     \vspace{-18pt}
%     %     \caption{PRECIPf48}
%     %     % \vspace{-9pt}
%     %     \label{fig:qnet_precip_ssim}
%     % \end{subfigure}
%     % \hfill
%     \begin{subfigure}{.49\columnwidth}
%         \includegraphics[width=\columnwidth]{Figures/sec-4/qnet_RTM420_SSIM.png}
%         \vspace{-18pt}
%         \caption{{RTM}}
%         % \vspace{-9pt}
%         \label{fig:qnet_seis_ssim}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{.49\columnwidth}
%         \includegraphics[width=\columnwidth]{Figures/sec-4/qnet_633_SSIM.png}
%         \vspace{-18pt}
%         \caption{{Density}}
%         % \vspace{-9pt}
%         \label{fig:qnet_density_ssim}
%     \end{subfigure}
%     \hfill
%     \vspace{-9pt}
%     \caption{SSIM prediction. \texttt{\_o} and \texttt{\_p} represent the ground truth and predicted values, respectively.}
%     \vspace{-5pt}
%     \label{fig:ssim_pred}
% \end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{subfigure}{.49\columnwidth}
        \includegraphics[width=\columnwidth]{Figures/sec-4/qnet_APE_BD_PSNR.png}
        \vspace{-18pt}
        \caption{Nyx - Baryon density}
        % \vspace{-9pt}
        \label{fig:qnet_bd_psnr}
    \end{subfigure}
    % \hfill
    % \begin{subfigure}{.49\columnwidth}
    %     \includegraphics[width=\columnwidth]{Figures/sec-4/qnet_APE_DMD_PSNR.png}
    %     \vspace{-18pt}
    %     \caption{Dark matter density}
    %     % \vspace{-9pt}
    %     \label{fig:qnet_dmd_psnr}
    % \end{subfigure}
    % \hfill
    \begin{subfigure}{.49\columnwidth}
        \includegraphics[width=\columnwidth]{Figures/sec-4/qnet_APE_CLOUDf48_PSNR.png}
        \vspace{-18pt}
        \caption{Hurricane - CLOUDf48}
        % \vspace{-9pt}
        \label{fig:qnet_cloud_psnr}
    \end{subfigure}
    % \hfill
    % \begin{subfigure}{.49\columnwidth}
    %     \includegraphics[width=\columnwidth]{Figures/sec-4/qnet_APE_PRECIPf48_PSNR.png}
    %     \vspace{-18pt}
    %     \caption{PRECIPf48}
    %     % \vspace{-9pt}
    %     \label{fig:qnet_precip_psnr}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}{.49\columnwidth}
    %     \includegraphics[width=\columnwidth]{Figures/sec-4/qnet_APE_QCLOUDf48_PSNR.png}
    %     \vspace{-18pt}
    %     \caption{{QCLOUDf48}}
    %     % \vspace{-9pt}
    %     \label{fig:qnet_qcloud_psnr}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}{.49\columnwidth}
    %     \includegraphics[width=\columnwidth]{Figures/sec-4/qnet_APE_QGRAUPf48_PSNR.png}
    %     \vspace{-18pt}
    %     \caption{{QGRAUPf48}}
    %     % \vspace{-9pt}
    %     \label{fig:qnet_qgraup_psnr}
    % \end{subfigure}
    % \hfill
    \begin{subfigure}{.49\columnwidth}
        \includegraphics[width=\columnwidth]{Figures/sec-4/qnet_APE_633_PSNR.png}
        \vspace{-18pt}
        \caption{{Miranda - Density}}
        % \vspace{-9pt}
        \label{fig:qnet_minranda_psnr}
    \end{subfigure}
    % \hfill
    \begin{subfigure}{.49\columnwidth}
        \includegraphics[width=\columnwidth]{Figures/sec-4/qnet_APE_355_PSNR.png}
        \vspace{-18pt}
        \caption{{RTM - Seismic wavefield}}
        % \vspace{-9pt}
        \label{fig:qnet_rtm_psnr}
    \end{subfigure}
    % \hfill
    % \vspace{-12pt}
    \caption{\wang{PSNR prediction error.}}
    \vspace{-10pt}
    \label{fig:ape_psnr}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{subfigure}{0.49\columnwidth}
        \includegraphics[width=\columnwidth]{Figures/sec-4/qnet_APE_BD_ssim.png}
        \vspace{-18pt}
        \caption{Baryon density}
        % \vspace{-9pt}
        \label{fig:qnet_bd_ssim}
    \end{subfigure}
    % \hfill
    % \begin{subfigure}{0.49\columnwidth}
    %     \includegraphics[width=\columnwidth]{Figures/sec-4/qnet_APE_DMD_ssim.png}
    %     \vspace{-18pt}
    %     \caption{Dark matter density}
    %     % \vspace{-9pt}
    %     \label{fig:qnet_dmd_ssim}
    % \end{subfigure}
    % \hfill
    \begin{subfigure}{0.49\columnwidth}
        \includegraphics[width=\columnwidth]{Figures/sec-4/qnet_APE_CLOUDf48_ssim.png}
        \vspace{-18pt}
        \caption{CLOUDf48}
        % \vspace{-9pt}
        \label{fig:qnet_cloud_ssim}
    \end{subfigure}
    % \hfill
    % \begin{subfigure}{0.49\columnwidth}
    %     \includegraphics[width=\columnwidth]{Figures/sec-4/qnet_APE_PRECIPf48_ssim.png}
    %     \vspace{-18pt}
    %     \caption{PRECIPf48}
    %     % \vspace{-9pt}
    %     \label{fig:qnet_precip_ssim}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}{0.49\columnwidth}
    %     \includegraphics[width=\columnwidth]{Figures/sec-4/qnet_APE_QCLOUDf48_ssim.png}
    %     \vspace{-18pt}
    %     \caption{{QCLOUDf48}}
    %     % \vspace{-9pt}
    %     \label{fig:qnet_qcloud_ssim}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}{0.49\columnwidth}
    %     \includegraphics[width=\columnwidth]{Figures/sec-4/qnet_APE_QGRAUPf48_ssim.png}
    %     \vspace{-18pt}
    %     \caption{{QGRAUPf48}}
    %     % \vspace{-9pt}
    %     \label{fig:qnet_qgraup_ssim}
    % \end{subfigure}
    % \hfill
    \begin{subfigure}{0.49\columnwidth}
        \includegraphics[width=\columnwidth]{Figures/sec-4/qnet_APE_633_ssim.png}
        \vspace{-18pt}
        \caption{{Density}}
        % \vspace{-9pt}
        \label{fig:qnet_minranda_ssim}
    \end{subfigure}
    % \hfill
    \begin{subfigure}{0.49\columnwidth}
        \includegraphics[width=\columnwidth]{Figures/sec-4/qnet_APE_355_ssim.png}
        \vspace{-18pt}
        \caption{{Seismic wavefield}}
        % \vspace{-9pt}
        \label{fig:qnet_rtm_ssim}
    \end{subfigure}
    % \hfill
    % \vspace{-12pt}
    \caption{SSIM prediction error.}
    \vspace{-10pt}
    \label{fig:ape_ssim}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{subfigure}{0.49\columnwidth}
        \includegraphics[width=\columnwidth]{Figures/sec-4/qnet_APE_BD_CR.png}
        \vspace{-18pt}
        \caption{Baryon density}
        % \vspace{-9pt}
        \label{fig:qnet_bd_cr}
    \end{subfigure}
    % \hfill
    % \begin{subfigure}{0.49\columnwidth}
    %     \includegraphics[width=\columnwidth]{Figures/sec-4/qnet_APE_DMD_CR.png}
    %     \vspace{-18pt}
    %     \caption{Dark matter density}
    %     % \vspace{-9pt}
    %     \label{fig:qnet_dmd_cr}
    % \end{subfigure}
    % \hfill
    \begin{subfigure}{0.49\columnwidth}
        \includegraphics[width=\columnwidth]{Figures/sec-4/qnet_APE_CLOUDf48_CR.png}
        \vspace{-18pt}
        \caption{CLOUDf48}
        % \vspace{-9pt}
        \label{fig:qnet_cloud_cr}
    \end{subfigure}
    % \hfill
    % \begin{subfigure}{0.49\columnwidth}
    %     \includegraphics[width=\columnwidth]{Figures/sec-4/qnet_APE_PRECIPf48_CR.png}
    %     \vspace{-18pt}
    %     \caption{PRECIPf48}
    %     % \vspace{-9pt}
    %     \label{fig:qnet_precip_cr}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}{0.49\columnwidth}
    %     \includegraphics[width=\columnwidth]{Figures/sec-4/qnet_APE_QCLOUDf48_CR.png}
    %     \vspace{-18pt}
    %     \caption{{QCLOUDf48}}
    %     % \vspace{-9pt}
    %     \label{fig:qnet_qcloud_cr}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}{0.49\columnwidth}
    %     \includegraphics[width=\columnwidth]{Figures/sec-4/qnet_APE_QGRAUPf48_CR.png}
    %     \vspace{-18pt}
    %     \caption{{QGRAUPf48}}
    %     % \vspace{-9pt}
    %     \label{fig:qnet_qgraup_cr}
    % \end{subfigure}
    % \hfill
    \begin{subfigure}{0.49\columnwidth}
        \includegraphics[width=\columnwidth]{Figures/sec-4/qnet_APE_633_CR.png}
        \vspace{-18pt}
        \caption{{Density}}
        % \vspace{-9pt}
        \label{fig:qnet_minranda_cr}
    \end{subfigure}
    % \hfill
    \begin{subfigure}{0.49\columnwidth}
        \includegraphics[width=\columnwidth]{Figures/sec-4/qnet_APE_355_CR.png}
        \vspace{-18pt}
        \caption{{Seismic wavefield}}
        % \vspace{-9pt}
        \label{fig:qnet_rtm_cr}
    \end{subfigure}
    % \hfill
    % \vspace{-12pt}
    \caption{CR prediction error.}
    \vspace{-10pt}
    \label{fig:ape_cr}
\end{figure*}
